The Authors Matter: Understanding and Mitigating Implicit Bias in Deep Text Classification

It is evident that deep text classification models trained on human data could be biased. In particular, they produce biased outcomes for texts that explicitly include identity terms of certain demographic groups. We refer to this type of bias as explicit bias, which has been extensively studied. However, deep text classification models can also produce biased outcomes for texts written by authors of certain demographic groups. We refer to such bias as implicit bias of which we still have a rather limited understanding. In this paper, we first demonstrate that implicit bias exists in different text classification tasks for different demographic groups. Then, we build a learning-based interpretation method to deepen our knowledge of implicit bias. Specifically, we verify that classifiers learn to make predictions based on language features that are related to the demographic attributes of the authors. Next, we propose a framework Debiased-TC to train deep text classifiers to make predictions on the right features and consequently mitigate implicit bias. We conduct extensive experiments on three real-world datasets. The results show that the text classification models trained under our proposed framework outperform traditional models significantly in terms of fairness, and also slightly in terms of classification performance.

==> backup.tex <==
\begin{table*}[t]
\small
\centering
\caption{Preliminary study.}
\label{tab:prelim}
\begin{tabular}{cccccccccccc}
% \hline
% \hline
% \multicolumn{6}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Twitter \end{tabular}}}\\
\hline
\hline
\multirow{2}{1cm}{\textbf{Dataset}} & \multirow{2}{1cm}{\textbf{Task}} & \multirow{2}{1cm}{\textbf{Demo}} & \multicolumn{3}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}False Positive (\%) \end{tabular}}} & \multicolumn{3}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}False Negative (\%) \end{tabular}}} & \multicolumn{3}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Demographic Parity (\%) \end{tabular}}} \\ \cmidrule(r){4-6}  \cmidrule(r){7-9} \cmidrule(r){10-12}
 & & & \textbf{Group I} & \textbf{Group II} & \textbf{FPED} & \textbf{Group I} & \textbf{Group II} & \textbf{FNED} & \textbf{Group I} & \textbf{Group II} & \textbf{DPD} \\ \hline
\multirow{2}{1cm}{\textbf{DIAL}} & \textbf{Sentiment} & \textbf{Race} & 46.29 & 27.40 & 18.89 & 23.13 & 61.48 & 38.34 & 61.58 & 32.96 & 28.62 \\
 & \textbf{Mention} & \textbf{Race} & 46.51 & 14.98 & 31.53 & 17.32 & 35.47 & 18.15 & 64.59 & 39.76 & 24.84 \\
 \hline
\multirow{2}{1cm}{\textbf{PAN16}} & \textbf{Mention} & \textbf{Gender} & 18.73 & 9.16 & 9.57 & 16.22 & 27.13 & 10.91 & 51.26 & 41.02 & 10.24 \\
 & \textbf{Mention} & \textbf{Age} & 26.93 & 11.32 & 15.60 & 14.91 & 25.09 & 10.18 & 56.01 & 43.12 & 12.89 \\
 \hline
\multirow{2}{1cm}{\textbf{MTC}} & \textbf{Hate Speech} & \textbf{Race} & 93.17 & 4.36 & 88.81 & 4.48 & 32.16 & 27.68 & 94.35 & 36.10 & 58.24 \\
& \textbf{Hate Speech} & \textbf{Gender} & 76.89 & 1.86 & 75.03 & 12.35 & 36.12 & 23.77 & 82.27 & 32.87 & 49.40 \\
\hline
\hline

\end{tabular}
\end{table*}


\begin{table*}[t]
\small
\centering
\caption{Text Classification Performance Comparison.}
\label{tab:performance}
\begin{tabular}{ccccccccccccc}
% \hline
% \hline
% \multicolumn{6}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Twitter \end{tabular}}}\\
\hline
\hline
\multirow{3}{1cm}{\textbf{Methods}} & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Sentiment|Race \end{tabular}}} & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Mention|Race \end{tabular}}} & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Mention|Gender \end{tabular}}} & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Mention|Age \end{tabular}}} & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Hate Speech|Race \end{tabular}}} & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Hate Speech|Gender \end{tabular}}}\\
 & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}(DIAL) \end{tabular}}} & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}(DIAL) \end{tabular}}} & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}(PAN16) \end{tabular}}} & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}(PAN16) \end{tabular}}} & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}(MTC) \end{tabular}}} & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}(MTC) \end{tabular}}}\\ \cmidrule(r){2-3}  \cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(r){8-9} \cmidrule(r){10-11} \cmidrule(r){12-13}
 & \textbf{Acc. (\%)} & \textbf{F1 (\%)} & \textbf{Acc. (\%)} & \textbf{F1 (\%)} & \textbf{Acc. (\%)} & \textbf{F1 (\%)} & \textbf{Acc. (\%)} & \textbf{F1 (\%)} & \textbf{Acc. (\%)} & \textbf{F1 (\%)} & \textbf{Acc. (\%)} & \textbf{F1 (\%)}\\ \hline
 & \multicolumn{12}{c}{\textbf{\begin{tabular}[c]{@{}c@{}} CNN \end{tabular}}}\\
\hline
\textbf{Base Model} & 61.40 & 60.03 & 70.77 & 71.65 & 81.93 & 81.94 & 80.57 & 80.17 & 64.10 & 65.86 & 66.93 & 69.84 \\ %\hline
 \textbf{Data Aug} & 67.58 & 71.53 & 76.42 & 76.03 & 84.11 & 84.31 & 84.08 & 84.36 & 66.96 & 71.10 & 67.26 & 71.40 \\ %\hline
\textbf{Ins Weigh} & 61.06 & 60.36 & 71.62 & 69.66 & 81.86 & 81.85 & 80.70 & 81.05 & 65.25 & 68.73 & 66.27 & 68.58\\ %\hline
\textbf{Debiased-TC} & 63.60 & 67.15 & 73.52 & 72.23 & 81.98 & 81.48 & 81.11 & 80.54 & 65.52 & 67.73 & 64.08 & 65.36\\ %\hline
\hline
 & \multicolumn{12}{c}{\textbf{\begin{tabular}[c]{@{}c@{}} RNN \end{tabular}}}\\ \hline
\textbf{Base Model} & 61.23 & 61.53 & 72.97 & 73.68 & 83.46 & 83.40 & 82.78 & 82.43 & 66.31 & 69.57 & 67.36 & 68.86\\ %\hline
 \textbf{Data Aug} & 67.82 & 69.35 & 78.42 & 77.26 & 86.25 & 86.05 & 86.12 & 85.68 & 68.55 & 72.37 & 68.46 & 72.65\\ %\hline
\textbf{Ins Weigh} & 61.23 & 61.53 & 73.37 & 73.79 & 83.46 & 83.32 & 82.80 & 82.58 & 67.26 & 70.94 & 66.43 & 68.04\\ %\hline
\textbf{Debiased-TC} & 64.06 & 66.47 & 74.73 & 73.56 & 81.30 & 81.33 & 81.55 & 81.20 & 63.66 & 63.88 & 66.97 & 70.24\\ %\hline
\hline
\hline

\end{tabular}
\end{table*}

==> fairness_results_with_BERT.tex <==
\begin{table*}[t]
\small
\centering
\caption{Fairness evaluation.}
\label{tab:fairness}
\begin{tabular}{c|cccccccccc}
% \hline
% \hline
% \multicolumn{6}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Twitter \end{tabular}}}\\
\hline
\hline
\multirow{2}{1cm}{\textbf{Task}} & \multirow{2}{1cm}{\textbf{Methods}} & \multicolumn{3}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}CNN \end{tabular}}} & \multicolumn{3}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}RNN \end{tabular}}} & \multicolumn{3}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}BERT \end{tabular}}} \\ \cmidrule(r){3-5}  \cmidrule(r){6-8}  \cmidrule(r){9-11}
 & & \textbf{FPED (\%)} & \textbf{FNED (\%)} & \textbf{DPD (\%)} & \textbf{FPED (\%)} & \textbf{FNED (\%)} & \textbf{DPD (\%)} & \textbf{FPED (\%)} & \textbf{FNED (\%)} & \textbf{DPD (\%)}\\ \hline
 & \textbf{Base Model} & 18.89 & 38.34 & 28.62 & 26.86 & 42.36 & 34.61 & - & - & - \\ \cmidrule(r){2-11}
\textbf{Sentiment} & \textbf{Data Aug} & 18.59 & 0.30 & 9.44 & 19.86 & 0.59 & 10.23 & - & - & -  \\
\textbf{Race} & \textbf{Ins Weigh} & 25.38 & 44.02 & 34.70 & 26.83 & 42.36 & 34.60 & - & - & -  \\ \cmidrule(r){2-11} %\hline 
\textbf{(DIAL)} & \textbf{Ours (Sup)} & - & - & - & - & - & - & - & - & -  \\ %\hline
 & \textbf{Ours} & - & - & - & - & - & - & - & - & -  \\ %\hline
\hline
\hline
 & \textbf{Base Model} & 31.53 & 18.15 & 24.84 & 29.85 & 16.30 & 23.07 & - & - & - \\ \cmidrule(r){2-11} %\hline
\textbf{Mention} & \textbf{Data Aug} & 0.80 & 7.14 & 3.17 & 0.53 & 7.49 & 4.01 & - & - & -  \\ %\hline
\textbf{Race} & \textbf{Ins Weigh} & 27.85 & 17.75 & 22.80 & 28.81 & 17.52 & 23.16 & - & - & -  \\ \cmidrule(r){2-11} %\hline 
\textbf{(DIAL)} & \textbf{Ours (Sup)} & - & - & - & - & - & - & - & - & -  \\ %\hline
 & \textbf{Ours} & - & - & - & - & - & - & - & - & - \\ %\hline
\hline
\hline
 & \textbf{Base Model} & 9.57 & 10.91 & 10.24 & 12.44 & 9.38 & 10.91 & - & - & - \\ \cmidrule(r){2-11} %\hline
\textbf{Mention} & \textbf{Data Aug} & 1.91 & 0.98 & 0.47 & 2.75 & 0.22 & 1.48 & - & - & -  \\ %\hline
\textbf{Gender} & \textbf{Ins Weigh} & 9.83 & 10.00 & 9.92 & 11.89 & 8.42 & 10.16 & - & - & -  \\ \cmidrule(r){2-11} %\hline 
\textbf{(PAN16)} & \textbf{Ours (Sup)} & - & - & - & - & - & - & - & - & -  \\ %\hline
 & \textbf{Ours} & - & - & - & - & - & - & - & - & - \\ %\hline
\hline
\hline
 & \textbf{Base Model} & 15.60 & 10.18 & 12.89 & 13.41 & 6.65 & 10.03 & - & - & - \\ \cmidrule(r){2-11} %\hline
\textbf{Mention} & \textbf{Data Aug} & 3.26 & 1.97 & 0.65 & 1.99 & 3.04 & 0.52 & - & - & -  \\ %\hline
\textbf{Age} & \textbf{Ins Weigh} & 16.28 & 8.81 & 12.54 & 11.82 & 7.19 & 9.51 & - & - & -  \\ \cmidrule(r){2-11} %\hline 
\textbf{(PAN16)} & \textbf{Ours (Sup)} & - & - & - & - & - & - & - & - & -  \\ %\hline
 & \textbf{Ours} & - & - & - & - & - & - & - & - & - \\ %\hline
\hline
\hline
 & \textbf{Base Model} & 88.81 & 27.68 & 58.24 & 81.15 & 31.68 & 56.42 & - & - & - \\ \cmidrule(r){2-11} %\hline
\textbf{Hate Speech} & \textbf{Data Aug} & 90.93 & 21.20 & 56.07 & 83.63 & 26.15 & 54.89 & - & - & -  \\ %\hline
\textbf{Race} & \textbf{Ins Weigh} & 82.10 & 39.34 & 60.72 & 83.98 & 33.69 & 58.83 & - & - & -  \\ \cmidrule(r){2-11} %\hline 
\textbf{(MTC)} & \textbf{Ours (Sup)} & - & - & - & - & - & - & - & - & -  \\ %\hline
 & \textbf{Ours} & - & - & - & - & - & - & - & - & - \\ %\hline
\hline
\hline
 & \textbf{Base Model} & 75.03 & 23.77 & 49.40 & 68.13 & 24.83 & 46.48 & - & - & - \\ \cmidrule(r){2-11} %\hline
\textbf{Hate Speech} & \textbf{Data Aug} & 84.59 & 23.37 & 53.98 & 84.99 & 23.11 & 54.05 & - & - & -  \\ %\hline
\textbf{Gender} & \textbf{Ins Weigh} & 78.35 & 24.17 & 51.26 & 76.49 & 29.35 & 52.92 & - & - & -  \\ \cmidrule(r){2-11} %\hline 
\textbf{(MTC)} & \textbf{Ours (Sup)} & - & - & - & - & - & - & - & - & -  \\ %\hline
 & \textbf{Ours} & - & - & - & - & - & - & - & - & - \\ %\hline
\hline
\hline


\end{tabular}
\vspace{-3pt}
\end{table*}

\begin{table*}[t]
\small
\centering
\caption{Performance comparision. \haochen{May need to replace this table with a figure.}}
\label{tab:performance}
\begin{tabular}{ccccccccc}
% \hline
% \hline
% \multicolumn{6}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Twitter \end{tabular}}}\\
\hline
\hline
\multirow{2}{1cm}{\textbf{Task}} & \multirow{2}{1cm}{\textbf{Demo}} & \multirow{2}{1cm}{\textbf{Methods}} & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}CNN \end{tabular}}} & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}RNN \end{tabular}}} & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}BERT \end{tabular}}} \\ \cmidrule(r){4-5}  \cmidrule(r){6-7}  \cmidrule(r){8-9}
 & & & \textbf{Acc. (\%)} & \textbf{F1 (\%)} & \textbf{Acc. (\%)} & \textbf{F1 (\%)} & \textbf{Acc. (\%)} & \textbf{F1 (\%)} \\ \hline
\multirow{4}{1cm}{\textbf{Sentiment}} & \multirow{4}{1cm}{\textbf{Race}} & \textbf{Base Model} & 60.43 & 59.32 & 61.23 & 61.53 & - & - \\ %\hline
 & & \textbf{DA} & 67.17 & 70.48 & 67.81 & 69.35 & - & - \\ %\hline
 & & \textbf{Instance Weighting} & 61.13 & 59.79 & 61.23 & 61.53 & - & - \\ %\hline
 & & \textbf{Ours} & - & - & - & \textbf{-} & \textbf{-} & - \\ %\hline
\hline
\hline
\multirow{4}{1cm}{\textbf{Mention}} & \multirow{4}{1cm}{\textbf{Race}} & \textbf{Base Model} & 71.43 & 72.04 & 73.05 & 74.09 & - & - \\ %\hline
 & & \textbf{DA} & 76.51 & 75.72 & 78.26 & 77.18 & - & - \\ %\hline
 & & \textbf{Instance Weighting} & 71.33 & 70.99 & 73.42 & 73.81 & - & - \\ %\hline
 & & \textbf{Ours} & - & - & - & \textbf{-} & \textbf{-} & - \\ %\hline
\hline
\hline

\end{tabular}
\vspace{-3pt}
\end{table*}

==> problem.tex <==
\section{Problem Statement}
\label{sec:problem}

In our text classification tasks, we denote a text as $X$, its ground-truth label as $Y$, and the demographic attribute of the author of the text as $Z$. The text $X$ consists of a sequence of words denoted as $(x_1, x_2, \dots, x_n)$, where $x_i$ is the $i$-th word in the text and $n$ is the length of the text. $Y$ and $Z$ are categorical labels with multiple possible values, such as ``positive'' and ``negative'' for $Y$ in a sentiment analysis task, and ``male'' and ``female'' for $Z$ \footnote{In this work, we consider only binary labels for $Y$ and $Z$ for simplicity. All the methodology and conclusions can be easily extended to the case of multiple labels.}. A text classifier attempts to accurately classify an input text into the correct category. It can be viewed as a function $\mathcal{M}:X\rightarrow Y$ that maps the text $X$ to label $Y$. A text classification model without implicit bias should make the prediction based on only the semantic information of a text and disregard the demographic attribute of its author. Thus, we seek to build a fair text classification model that makes prediction $\hat{Y}$ independent of $Z$ in terms of certain fairness evaluation metrics.

We use the following evaluation metrics to measure the fairness of a text classification model in terms of implicit bias: 1) False Positive/Negative Equality Differences \cite{dixon2018measuring} and 2) Demographic Parity Difference \cite{dwork2012fairness,kusner2017counterfactual}. The False Positive/Negative Equality Differences (FPED/FNED) are defined as

\begin{align}
    FPED &= \sum_{\forall Z} |FPR_{Z} - FPR_{overall}| \nonumber\\
    FNED &= \sum_{\forall Z} |FNR_{Z} - FNR_{overall}| \nonumber
\end{align}

\noindent where $FPR_{Z}$ and $FNR_{Z}$ denote the false positive rate and the false negative rate of texts with demographic attribute $Z$ respectively, while $FPR_{overall}$ and $FNR_{overall}$ are the false positive rate and the false negative rate of the texts with all the demographic attributes, respectively. Demographic Parity suggests that a fair classifier should assign a positive label to texts produced by both demographic groups with equal probability. Demographic Parity Difference is defined as below.
\begin{align}
    DPD = |P(\hat{Y}=1|Z=0) - P(\hat{Y}=1|Z=1)| \nonumber
\end{align}
A text classification model free from implicit bias makes predictions independent of demographic attributes. Thus, it should have similar false positive and negative rates for both demographic groups and also satisfies demographic parity, which implies small FPED/PNED and DPD.
 

% \begin{align}
%     EOD = |P(\hat{Y}=1|Z=0,Y=1) - P(\hat{Y}=1|Z=1,Y=1)| \nonumber
% \end{align}
% The $\mathbf{T}=\{X_i, Y_i, Z_i\}_{i=1}^N$. 
